Reflectance study of ice and Mars soil simulant associations -- I. H$_2$O ice

The reflectance of water ice and dust mixtures depends, amongst other parameters, on how the components are mixed (e.g. intimate mixture, areal mixture or coating) (Clark et al. 1999). Therefore, when inverting the reflectance spectra measured from planetary surfaces to derive the amount of water ice present at the surface, it is critical to distinguish between different mixing modes of ice and dust. However, the distinction between mixing modes from reflectance spectra remains ambiguous. Here we show how to identify some water ice/soil mixing modes from the study of defined spectral criteria and colour analysis of laboratory mixtures. We have recreated ice and dust mixtures and found that the appearance of frost on a surface increases its reflectance and flattens its spectral slopes, whereas the increasing presence of water ice in intimate mixtures mainly impacts the absorption bands. In particular, we provide laboratory data and a spectral analysis to help interpret ice and soil reflectance spectra from the Martian surface.

==> Intro.tex <==
\section{Introduction}
\label{S:1}

Reflectance spectroscopy is one of the techniques of choice to retrieve the physical properties of planetary surfaces from remote sensing \citep{NASAworkshop}. The study of the reflectance of a surface provides information about ---amongst others--- its composition, albedo, or size distribution of its particles, if relevant. Usually, ice on planetary surfaces is not pure but contaminated by other ices or minerals to different extents depending on the hosting body \citep{Clark_1984, Gianrico}. 

%This is, for instance, how the composition of icy planetary surfaces was discovered more than 40 years ago (\citep{Clark_1984} and references therein), or how we detect water ice in bodies of the Solar System nowadays, e.g., \citet{Gianrico}.

The shape of the reflectance spectrum of a mixture of water ice with other components depends on many parameters: the relative abundance of water ice, the albedo of the other elements of the mix, the mixing style, etc. Therefore, the inversion of acquired spectra is not unique unless many of these parameters are known beforehand. 

To understand how the way in which ice and dust are mixed influences the reflectance of the mixture, we have measured the visible (VIS) and near-infrared (NIR) reflectance of different ice and regolith mixtures (e.g., frost, intimate mixtures) at the Laboratory for Outflow Studies of Sublimating icy materials (LOSSy) \citep{Pommerol:2019} of the University of Bern. We have defined spectral and colour criteria and observed how they changed as the relative abundance of water ice increased. Then, we have looked for discriminative photometric signatures of each mixing mode. We have as well examined in which conditions discrete occurrences of water ice can be distinguished from hydrated minerals.

This paper proposes empirical methods to distinguish between ice-dust mixing modes from their visible colours and visible-near-infrared reflectance. We want to provide the scientific teams of current and past Martian missions with laboratory data comparable to the photometric data that have been or are being retrieved from the surface of Mars. Our intention is to help these teams fully exploit their data by comparing them to well characterised icy mixtures. We also intend to complement other laboratory work carried out to understand the influence of specific parameters in the reflectance spectra; for example, Kieffer and Clark in the 1970s and 1980s (e.g.\citet{Kieffer:1970, Clark_1984}) or Pommerol et al. more recently (e.g., \citet{Pommerol:2008}). This is the first of two publications about laboratory reflectance studies of ice and dust mixtures aiming at reproducing putative icy surfaces of Mars. While in this article we only present experiments with H$_2$O ice, we incorporate CO$_2$ ice to our study in the companion paper.

In the next section, we provide an overview of the presence of water ice at the surface of Mars. We also present previous laboratory work that has been carried out related to the icy Martian surfaces. We present in Section \ref{S:3} the materials, instruments, and methods that we have used in this study. In Section \ref{S:4} we show the results of our work, which we discuss in Section \ref{S:5}. Finally, Section \ref{S:7} summarises our work and gives further perspectives. 







==> Intro_Mars.tex <==
\section{Water ice on Mars. Laboratory work background.}
\label{S:intromars}

Over the last 4 billion years, the surface of Mars has undergone changes caused by volatile transport. It is now thought that water ice once covered low latitudes \citep{Head2003} and that the planet may have hosted a global ocean \citep{PARKER1987}. Nevertheless, the current conditions of pressure and temperature at ground level allow water to be present only in its solid or gaseous phase. Hence, water remains today trapped as ground ice (permafrost), stored in hydrated minerals, as sub-permafrost groundwater, and trapped in the polar caps. A review of the Martian hydrosphere, listing and quantifying the possible amounts of water within known and putative reservoirs, can be found in \citet{Lasue2013}. Here, we focus on the different ways in which ice and dust appear mixed on the Martian surface.

Because of the equilibrium vapour pressure of ice, there are traces of water vapour in the atmosphere. The concentration of water vapour in the Martian atmosphere varies considerably through the seasons (\citet{PANKINE2015107} and references therein). Diurnal variations of atmospheric water vapour have also been observed as water condenses as frost on the surface during cold nights and sublimes in the morning \citep{JGRB:JGRB7366}. This nighttime deposition of frost can occur at low latitudes: \citet{Carrozzo:2009} reported frost depositions between 30$^\circ$N and 30$^\circ$S) and \citet{MARTINEZ201693} identified a micrometric layer of frost on the surface of Gale crater (5.6$^\circ$S).

Water ice can also be found in the subsurface as permafrost, an ice-rich layer that spreads from 60$^\circ$S to 45$^\circ$N. Even though subsurface-ice is not accessible to imagers in the visible and near-infrared, it has been observed when exposed in impacts craters \citep{Byrne:2009,Dundas:2014}, excavated by the Phoenix mission \citep{Smith:2009} or at pits \citep{Dundas:2018}. Another example of exposed water ice and dust mixtures on Mars are the North Polar Layered Deposits (NPLD), a succession of almost horizontal layers of different ice and dust content \citep{Murray:1972}.  

Quantifying the ice on the surface is a crucial step in assessing the actual budgets of water on Mars. It also has repercussions for the overall energy balance ---a key aspect of the climate of the planet, since it changes the albedo of the surface. Hence, many research groups have already conducted laboratory campaigns to study the interaction between atmospheric water and the surface. For instance, \citet{GRL:GRL22559} studied the sublimation rate of water ice under simulated Mars conditions and found that a one-meter thick layer of water ice underneath a meter of Martian regolith would last around 800 years (at a temperature of 235 K). Also simulating Martian conditions (i.e., the same range of pressure and temperature but higher water concentration in the atmosphere), \citet{JGRE:JGRE2537} showed that atmospheric water could condense as subsurface ice. \citet{Kaufmann:2015} studied the penetration of solar radiation into both pure and Mars-dust contaminated snow and pointed out the major role played by small-scale inhomogeneities in the way light penetrates an ice-dust mixture.

Even though techniques such as reflectance spectrometry and photometry are often used on Mars to look for changes in surface reflectance and to identify ice (e.g., \citet{Kieffer:70}, \citet{Langevin2007}), there is a lack of experimental data on the reflectance of water ice and dust mixtures. Back in 1981, \citet{Clark:1981} measured the reflectance of water frost grown on Mauna Kea red cinder in the laboratory and noted a distinct effect of frost in the VIS and NIR parts of the spectrum. In 2013, \citet{JGRE:JGRE20158} studied the bidirectional reflectance of dry, wet and frozen Martian regolith analogues and showed that the photometric signatures of their icy samples depended mostly on the physical properties of the ice. More recently, \citet{Gyalay:2019} have measured the reflectance of intimate mixtures of water ice and JSC Mars-1 in the range of 400-1000 nm. Nevertheless, some fundamental aspects such as the influence on the reflectance spectra of the type of mixture between the soil and the ice have not been fully explored, even though such data are key for a correct interpretation of orbital data and calibration of reflectance models. 

We aim to broaden the laboratory characterisation of Martian, icy soil analogues by providing a spectral and colour study of various Martian-like regolith and ice mixtures prepared in a controlled way. Furthermore, we provide laboratory data comparable in spectral range and resolution with those acquired by instruments observing Mars from orbit, e.g. imaging spectrometers like Observatoire pour la Min{\'e}ralogie, l'Eau, les Glaces et l’Activit{\'e} (OMEGA) \citep{Bibring:Omega} or Compact Reconnaissance Imaging Spectrometer for Mars (CRISM) \citep{Murchie:2007}, and colour imagers such as the High-Resolution Stereo Camera (HRSC) \citep{Jaumann:2007}, High Resolution Imaging Science Experiment (HiRISE) \citep{McEwen:2007}, or the Colour and Stereo Surface Imaging System (CaSSIS) \citep{Thomas2017}. Of particular interest for us is CaSSIS, the camera on board ESA's Trace Gas Orbiter (TGO), since it complements the data of HRSC and HiRISE thanks to its high signal-to-noise ratio (SNR) and the non-Sun-synchronous orbit of TGO. This orbit is of particular interest for frost detection, because it allows us to observe not only seasonal phenomena but also diurnal ones. For this reason, we use as colours of reference CaSSIS' four bands BLU, PAN, RED and NIR (which have their nominal effective centre at 485, 675, 840 and 985 nm respectively \citep{Thomas2017}).





